Egocentric Vision-based Future Vehicle Localization for Intelligent Driving Assistance Systems

Predicting the future location of vehicles is essential for safety-critical applications such as advanced driver assistance systems (ADAS) and autonomous driving. This paper introduces a novel approach to simultaneously predict both the location and scale of target vehicles in the first-person (egocentric) view of an ego-vehicle. We present a multi-stream recurrent neural network (RNN) encoder-decoder model that separately captures both object location and scale and pixel-level observations for future vehicle localization. We show that incorporating dense optical flow improves prediction results significantly since it captures information about motion as well as appearance change. We also find that explicitly modeling future motion of the ego-vehicle improves the prediction accuracy, which could be especially beneficial in intelligent and automated vehicles that have motion planning capability. To evaluate the performance of our approach, we present a new dataset of first-person videos collected from a variety of scenarios at road intersections, which are particularly challenging moments for prediction because vehicle trajectories are diverse and dynamic.

==> ProblemDataset.tex <==
\section{Problem Formulation and First-person View Intersection Dataset}
\subsection{Problem Formulation}
Our goal is to predict the future bounding boxes of vehicles in the future frames of a front-view camera. This is different from the traditional trajectory prediction because the location and scale of objects in camera frame doesn't correspond to physical location directly. 

The past trajectory of a vehicle is defined as $\mathbf{X}=\{X_{t-\tau+1},X_{t-\tau+2},...,X_t\}$, where $X_t=[x_t,y_t,w_t,h_t]$ contains the pixel coordinates of the vehicle bounding box at time $t$ together with its width and height in pixels. Similarly, the future trajectory of the bounding box is defined as $\mathbf{Y}=\{Y_{t+1},Y_{t+2},...,Y_{t+\delta}\}$.
Given $\mathbf{O}=\{O_{t-\tau+1},O_{t-\tau+2},...,O_t\}$ the image evidences observed from the past $\tau$ frames, the goal is to predict the future bounding boxes $\mathbf{Y}$. % that maximize the posterior 



% \begin{equation}
%     \hat{\mathbf{Y}} = \argmax_{Y}\, {P(\mathbf{Y}|\mathbf{X}, \mathbf{O})}
% \end{equation}

\subsection{Front View Intersection Dataset}
The proposed future vehicle localization problem especially focuses on scenarios where the object vehicles operate diverse motions. However, to the best of our knowledge, most of the existing driving datasets are proposed for object detection, tracking or scene understanding purpose, which doesn't contain sufficient amount of motions. In this paper, we propose a new data set contains large amount of first-person video frames where many object vehicles proceed with diverse motions.

The proposed first-person view intersection dataset contains $230$ video clips collected from different types of intersections with length varying from $10$ seconds to $1$ minutes. Videos are collected from a camera mounted on the wind-shield of a moving car, with $1920\times 1200$ resolution and $10\, fps$. We select intersections as the data collection area since most of the complicated object-host vehicles interactions are found at intersections.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width = 1\columnwidth]{Figures/dataset/dataset_1.png}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width = 1\columnwidth]{Figures/dataset/dataset_3.png}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width = 1\columnwidth]{Figures/dataset/dataset_4.png}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.48\columnwidth}
        \centering
        \includegraphics[width = 1\columnwidth]{Figures/dataset/dataset_5.png}
    \end{subfigure}
    \caption{Front-view Vehicle Localization Dataset. }
    \label{fig:dataset}
\end{figure}

The FVL data set is constructed following a pipeline similar to \cite{yagi2017future}. For each video, we detect and track each object vehicle and select vehicles last for more than $20$ frames ($2$ seconds). The training and testing samples are generated by a timing window with length $20$ so that the input and output lengths are $T_{in} = T_{out} = 10$.

There are more than $2,400$ vehicle tracklets 

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
        Data set & \# videos & \# tracklets & scene types  \\
        \hline
        KITTI & & & \\
        Cityscapes & & & \\
        Ours & & &
    \end{tabular}
    \caption{Comparison with other data sets}
    \label{tab:datasets}
\end{table}

Note that this dataset also comes with synchronized LiDAR data as well as IMU, GPS and CAN Bus signals. In this paper, we only use the first-person video to provide benchmarks for vision based future location prediction. In future, depth and road layout information (LiDAR, GPS) can be included to make a more informative traffic scene prediction.


